The Inventory is Dark and Full of Misinformation: Understanding the Abuse of Ad Inventory Pooling in the Ad-Tech Supply Chain

Ad-tech enables publishers to programmatically sell their ad inventory to millions of demand partners through a complex supply chain. Bogus or low quality publishers can exploit the opaque nature of the ad-tech to deceptively monetize their ad inventory. In this paper, we investigate for the first time how misinformation sites subvert the ad-tech transparency standards and pool their ad inventory with unrelated sites to circumvent brand safety protections. We find that a few major ad exchanges are disproportionately responsible for the dark pools that are exploited by misinformation websites. We further find evidence that dark pooling allows misinformation sites to deceptively sell their ad inventory to reputable brands. We conclude with a discussion of potential countermeasures such as better vetting of ad exchange partners, adoption of new ad-tech transparency standards that enable end-to-end validation of the ad-tech supply chain, as well as widespread deployment of independent audits like ours.

==> ethics.tex <==
%%
We discuss the ethics of our web crawling along three dimensions: infrastructure costs, privacy risks, and advertising costs caused by this study.

%%
\parait{Infrastructure costs.} Our crawling methodology was used only for measuring the prevalence of compliance issues and misrepresentations to understand its effect on brands. 
%
Our two dynamic crawls were not conducted concurrently to avoid stress on the website servers. 
%
Similarly, our additional static crawls for \ads and \sellers were performed six months apart. Our crawling mechanism was in line with the typical auditing studies as described in Sandvig et al.~\cite{sandvig2014auditing} and is not considered in violation of the CFAA.

%%
\parait{Privacy risks.} By visiting only the front pages of each website using full-fledged web browsers, our dynamic crawls did not disobey the robots.txt directives set by publishers. 
%
Additionally, our study did not involve human subjects or gather any personally identifiable information (PII).

%%
\parait{Advertising costs.} To actually understand what brands are advertising on misinformation websites and what ad-exchange is responsible for showing that ad, we had no other option but to explicitly click on the ads shown during the dynamic load of the websites because no public APIs are available to obtain this information. 
%
The dollar costs associated with our clicks are negligible (CPMs are in the order of cents and we clicked a total of 4247 ads). 
%
This negligible cost trade-off is necessary to understand vulnerabilities in ad-tech and the funding of online misinformation ecosystems.

%%
Overall, our study respects the principle of beneficence as outlined in the Menlo Report~\cite{MenloReport2012} and Belmont Report~\cite{BelmontReport1979} by maximizing the possible benefits and minimizing the harms.


==> metareview.tex <==
\vfill\eject
\section{Meta-Review}

\subsection{Summary}
This paper investigates how dark pooling of ad inventory leads to misrepresentation of the true property on which ads are displayed, bypassing brand safety measures used by major ad exchanges. The authors perform a large-scale measurement study to identify and characterize how this dark pooling leads to misinformation sites selling ads to major brands.

%

\subsection{Scientific Contributions}
%\yash{Should the letters be capitalized below?}
\begin{itemize}
\item Independent Confirmation of Important Results with Limited Prior Research
\item Provides a New Data Set For Public Use
\item Establishes a New Research Direction
\item Provides a Valuable Step Forward in an Established Field
\end{itemize}

%

\subsection{Reasons for Acceptance}
\begin{enumerate}
\item This paper provides independent confirmation of important results with limited prior research. While the issue of ad inventory misrepresentation was known, its prevalence was not well-characterized. The work’s large-scale measurement demonstrates the real-world impact of this issue.
\item The paper provides a new data set for public use and establishes a future research direction. Measurement study data is being shared in a format that will enable future analysis of ad inventory misrepresentation. New research in ad inventory transparency, including several suggested in the paper, can leverage this data.
\item The paper provides a valuable step forward in an established field. The paper provides a systematic review of the interaction between ad inventory transparency and the real-world behavior of advertisers and website operators.
\end{enumerate}

%

\subsection{Noteworthy Concerns} % Exclude if your meta-review does not have noteworthy concerns
\begin{enumerate} % Enumerate environment is not necessary if there is only one
\item The vulnerabilities discussed in the paper are not novel. It is already understood that ad standards are not effectively enforced and that dark pooling can undermine the validation of ad supply chains.
\item While this paper performed a detailed study on ad fraud, the measurement methodology is straightforward and not technically challenging.
\item Because detected advertisers are a lower-bound, some correlations presented in the paper may not hold if this undercounting is not uniform.
\item Because crawling was done from a single IP address, IP-based tracking could have biased measured advertisements.
\end{enumerate}

%

\begin{comment}

%\section{Response to the Meta-Review} % Optional

\yash{Please review the following response to meta-review:}

The advertising industry is already aware that the ad standards are not effectively enforced and that dark pooling can undermine the validation of ad supply chain. However, existence and prevalence of these issues is neither known nor scientifically studied. Additionally, the negative implications of these issues for buyers are unclear. Our study aims to bridge this gap by undertaking a standard internet measurement methodology to study this specific ad fraud.

We performed our crawls from a single IP-address. Assuming that advertising brands targeted ads to our crawler due to IP-based fingerprinting suggests there could have been a bias in our results. However, had ad we performed crawling from multiple IP addresses, we would have simply obtained more number of distinct brands. Using a single IP-address could not have biased the measured advertisements in any other way given that we perform crawl randomization and we crawl each website independently by spawning up a fresh browser with cleared cookies/storage (aka ``stateless crawl''). \yash{I am not sure how to address undercounting issue?}

\end{comment}

==> trust.tex <==
% Blurb for delegation of trust and trust vetting in PKI, play stores, etc. and parallels to this paper.
One of our key findings is that a small number of ad exchanges are responsible for a majority of dark pooling. In many cases, we see evidence that this dark pooling is achieved through the use of legitimate partner programs made available by ad exchanges (\eg Google's MCM partner program \cite{GoogleMCM}).
%
These programs serve an important purpose --- to help reduce the management burdens on small publishers. However, as we see in our study, this expanded access facilitated via advertising partners results in new vulnerabilities. Specifically, publishers who are in clear violation of the policies set by an ad exchange are still able to obtain seller IDs issued by the exchange through their partners.
%
One perspective of this problem is that there is a fundamental breakdown of trust delegation --- \ie partners are delegated the rights to assign and manage seller IDs on behalf of exchanges, but without being properly delegated the responsibilities for vetting publishers and verifying their compliance with ad exchange policies.
%
While this work is the first to uncover this delegation of trust in the form of verification responsibilities in the ad-tech ecosystem, it is not new to the security community. Indeed, this type of trust delegation is a central theme in the public key infrastructure, app stores, and other domains. 
%
From these prior efforts to delegate verification responsibilities, it is clear that success is only possible with effective mechanisms to monitor compliance and to revoke delegated trust. Unfortunately, it is not publicly known if these processes exist within specific ad exchanges.
%
Without public documentation of these processes or research studies that uncover them, we anticipate that identifying weaknesses and causes for failure will remain a challenge.
